Egocentric Network Exploration for Immersive Analytics

To exploit the potential of immersive network analytics for engaging and effective exploration, we promote the metaphor of "egocentrism", where data depiction and interaction are adapted to the perspective of the user within a 3D network. Egocentrism has the potential to overcome some of the inherent downsides of virtual environments, e.g., visual clutter and cyber-sickness. To investigate the effect of this metaphor on immersive network exploration, we designed and evaluated interfaces of varying degrees of egocentrism. In a user study, we evaluated the effect of these interfaces on visual search tasks, efficiency of network traversal, spatial orientation, as well as cyber-sickness. Results show that a simple egocentric interface considerably improves visual search efficiency and navigation performance, yet does not decrease spatial orientation or increase cyber-sickness. An occlusion-free Ego-Bubble view of the neighborhood only marginally improves the user's performance. We tie our findings together in an open online tool for egocentric network exploration, providing actionable insights on the benefits of the egocentric network exploration metaphor.

==> authors.tex <==
      
      \author[J. Sorger, A. Arleo, P. K\'{a}n, W. Knecht, M. Waldner]
{\parbox{\textwidth}{\centering J. Sorger\thanks{\{sorger|knecht\}@csh.ac.at}$^{1}$\orcid{0000-0002-5212-8941}
        , A. Arleo\thanks{\{alessio.arleo|kan|waldner\}@tuwien.ac.at}$^{2}$\orcid{0000-0003-2008-3651},
        P. K\'{a}n$^{\ddag23}$,
        W. Knecht$^{\dag1}$,
        and M. Waldner$^{\ddag2}$\orcid{0000-0003-1387-5132} 
        }
        \\
% For Computer Graphics Forum: Please use the abbreviation of your first name.
{\parbox{\textwidth}{\centering $^1$Complexity Science Hub Vienna, Austria
%- e-mail: \textit{sorger|knect@csh.ac.at}
\\
         $^2$TU Wien, Austria, 
         $^3$Aarhus University, Denmark
         %- e-mail: \textit{name.surname@tuwien.ac.at}
%        $^2$ Another Department to illustrate the use in papers from authors
%             with different affiliations
       } 
}
}
